Comparison of new computational methods for geostatistical modelling of malaria

Geostatistical analysis of health data is increasingly used to model spatial variation in malaria prevalence, burden, and other metrics. Traditional inference methods for geostatistical modelling are notoriously computationally intensive, motivating the development of newer, approximate methods. The appeal of faster methods is particularly great as the size of the region and number of spatial locations being modelled increases. Methods We present an applied comparison of four proposed `fast' geostatistical modelling methods and the software provided to implement them -- Integrated Nested Laplace Approximation (INLA), tree boosting with Gaussian processes and mixed effect models (GPBoost), Fixed Rank Kriging (FRK) and Spatial Random Forests (SpRF). We illustrate the four methods by estimating malaria prevalence on two different spatial scales -- country and continent. We compare the performance of the four methods on these data in terms of accuracy, computation time, and ease of implementation. Results Two of these methods -- SpRF and GPBoost -- do not scale well as the data size increases, and so are likely to be infeasible for larger-scale analysis problems. The two remaining methods -- INLA and FRK -- do scale well computationally, however the resulting model fits are very sensitive to the user's modelling assumptions and parameter choices. Conclusions INLA and FRK both enable scalable geostatistical modelling of malaria prevalence data. However care must be taken when using both methods to assess the fit of the model to data and plausibility of predictions, in order to select appropriate model assumptions and approximation parameters.

==> old_tables_and_figures.tex <==
% This contains the old tables where we used data for both species, and used iqrs and medians for INLA and SpRF. 

\begin{table}[!ht]
	\centering
	\caption{Cross validation results of the four models with best results in each category in boldface.}
	{
	\begin{tabular}{cp{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{2cm}}
		\toprule
  Model & 10-fold-RMSE &  50-fold RMSE & Training Correlation & 10-fold Correlation & 50-fold Correlation & \% points within 1SD/50P (10-fold)
   \\
        \midrule
       INLA    & 0.182  & 0.119  & 0.907  & 0.205   & 0.714 & 6.021 (50P)\\
     GPBoost   & \textbf{0.127} & \textbf{0.109} & 0.872 & \textbf{0.647}  & \textbf{0.754} & 69.11 (1SD) \\
     SpRF      & 0.131  &  0.121  & \textbf{0.909}  & 0.644 & 0.704 & 84.29 (50P) \\
     FRK       & 0.130  &  0.124  & 0.900 & 0.633 & 0.701  & 97.64 (1SD)\\
    \bottomrule
	\end{tabular} }
	\label{tab:predactualscv_old}
\end{table}


\begin{table}[!ht]
    \centering
    \caption{Times taken in minutes to train the models on each dataset and generate the prediction maps.  The \textit{Kenya: Observations} column corresponds to the maps in Figure~\ref{fig:Kenya_maps}. The \textit{Africa: Observations}, \textit{Africa: Simulated observations}, and \textit{Africa: Simulated uniform} columns correspond to columns (i), (ii), and (iii) of Figure~\ref{fig:Africa_prevalence_maps} respectively. Note that different machines were used for the Kenya and Africa datasets.}
    \begin{tabular}{cp{2cm}p{2cm}p{1.7cm}p{3cm}p{3cm}}
            \cmidrule{1-6}
           & & \multicolumn{4}{c}{Dataset} \\
           \cmidrule{3-6}
           & & Kenya: \mbox{Observation} &Africa: \mbox{Observation} & Africa: \mbox{Simulated} \mbox{observation}\ & Africa: \mbox{Simulated} \mbox{uniform} \\
           \cmidrule{1-6} \vspace{-5px}
           \\ 
           \multirow{4}{3em}{Model} & INLA & 0.41 & 48.53 & 7.21 & 9.70 \\
           & SpRF & 0.44 & 24.04 & 23.39 & 28.97\\
           & GPBoost & 1.16 & 13.30 & 8.75 & 13.38\\
           & FRK & 0.35 & 3.22 & 3.16 & 3.00 
           \vspace{5px}\\ 
           \cmidrule{1-6}
    \end{tabular}
    \label{tab:Map_times_old}
\end{table}



\begin{table}[!ht]
	\centering
	\caption{Cross validation results of the four models with best results in each category in boldface.}
	{
	\begin{tabular}{ccp{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
		\toprule
   \multirow{2}{*}{Fold} & \multirow{2}{*}{Model} & \multirow{2}{*}{RMSE}  & \multirow{2}{*}{Correlation} & \multicolumn{3}{c}{ \% points with absolute error less than } \\  % Absolute Error (\%)
   \cmidrule{5-7} & & &  & $ 0.05$ & $ 0.1$  & $  0.2$  \\
        \midrule
\multirow{4}{*}{10-fold}  
    &   INLA    & 0.182     &  0.205    & 68.848    & 76.702    & 86.126 \\
    & GPBoost   & \textbf{0.127}  &  \textbf{0.647} & 52.880    & 74.084 & \textbf{93.194} \\
    & SpRF      & 0.131     & 0.644     & \textbf{69.110}       & \textbf{80.890}  & 91.099 \\
    & FRK       & 0.130     &  0.633    & 58.155    & 71.990    &  91.361\\
        \midrule
\multirow{4}{*}{50-fold}  
    &   INLA    & 0.119     & 0.714 & \textbf{70.157}   & \textbf{80.890}   & 89.005 \\
& GPBoost & \textbf{0.109} & \textbf{0.754} & 65.969    & \textbf{80.890}   &  90.052\\
    & SpRF      & 0.121     &  0.704    & 68.063        & 79.319            & \textbf{90.314} \\
    & FRK       & 0.124     & 0.701     & 66.23         & 78.796            & 90.052\\        
		 \bottomrule
	\end{tabular} }
	\label{tab:predactuals_old}
\end{table}


\begin{table}[!ht]
	\centering
	\caption{Cross validation results grouped by density of sampled locations with best results in boldface.}
	{
	\begin{tabular}{cccp{1.3cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
		\toprule
   \multirow{2}{*}{Fold} & \multirow{2}{*}{Density} & \multirow{2}{*}{Model} & \multirow{2}{*}{RMSE}  & \multirow{2}{*}{Corr.} & \multicolumn{3}{c}{ \% points with absolute error less than } \\  % Absolute Error (\%)
   \cmidrule{6-8} & & & &  & $ 0.05$ & $ 0.1$  & $  0.2$  \\
        \midrule
\multirow{12}{*}{10-fold} & \multirow{4}{*}{Low}
    &   INLA    & \textbf{0.005}    & -0.223      & 100       & 100       & 100          \\
   &  & GPBoost & 0.025    & -0.182      & 96        & 100       & 100          \\
   &  & SpRF    & 0.005    & -0.046      & 100       & 100       & 100          \\
   &  & FRK     & 0.044    & -0.093      & 70        & 100       & 100          \\
   \cmidrule{2-8}
   & \multirow{4}{*}{Medium}
    &   INLA    & 0.14     & -0.001        & 76        & 83.429    & 93.714         \\
   &  & GPBoost & \textbf{0.138}     & -0.02         & 61.143    & 85.714    & 94.286         \\
   &  & SpRF    & 0.142     & -0.045        & 72        & 82.286    & 93.714         \\
   &  & FRK     & 0.151     & -0.057        & 60        & 66.286    & 92.571          \\
    \cmidrule{2-8}
    %\cdashline{2-8}
   & \multirow{4}{*}{High}
    &   INLA    & 0.242     & 0.273         & 50.955    & 61.783    & 73.248       \\
   &  & GPBoost & 0.134     & 0.788         & 29.936    & 52.866    & 89.809         \\
   &  & SpRF    & 0.139     & 0.742         & 56.051    & 73.248    & 85.35           \\
   &  & FRK     & \textbf{0.123}     & 0.809         & 52.229    & 69.427    & 87.261         \\
        \midrule 
        \midrule
        
\multirow{12}{*}{50-fold}  & \multirow{4}{*}{Low}
    &   INLA    & \textbf{0.005}     & -0.111        & 100       & 100       & 100     \\
  &  & GPBoost  & 0.015     & -0.202        & 100       & 100       & 100 \\
  &  & SpRF     & 0.006      & -0.076        & 100       & 100       & 100  \\
  &  & FRK      & 0.020     & -0.173        & 98        & 100       & 100 \\     
  \cmidrule{2-8}
  & \multirow{4}{*}{Medium}
     &   INLA   &  \textbf{0.110}    & 0.571         & 74.286    & 82.857    & 92.571        \\
  &  & GPBoost  &  0.115    & 0.516         & 73.143    & 84.571    & 92 \\
  &  & SpRF     &  0.120    &  0.437        & 72        & 86.286    & 96.571 \\
  &  & FRK      &  0.132    & 0.311         & 75.429    & 83.429    & 91.429\\
  \cmidrule{2-8}
   & \multirow{4}{*}{High}
     &   INLA   &   0.144    & 0.768         & 56.051    & 72.611    & 81.539\\
  &  & GPBoost  &   \textbf{0.119}   & 0.809         & 47.134    & 70.701    & 84.713 \\
  &  & SpRF     &   0.139   & 0.743         & 53.503    & 64.968    & 80.255 \\
  &  & FRK      &   0.133   & 0.779         & 45.86     & 66.879    & 85.35 \\  
		 \bottomrule
	\end{tabular} }
	\label{tab:predactualsdiffdensities_old}
\end{table}


\begin{table}[!ht]
	\centering
	\caption{Interval prediction results of the four models.}
	{
	\begin{tabular}{cccp{2.5cm}p{2.5cm}p{1.5cm}p{1.5cm}}
		\toprule
   \multirow{2}{*}{Fold} & \multirow{2}{*}{Model} & \multirow{2}{*}{Type}  & \multirow{2}*{\begin{tabular}{l} Mean \\ Width \end{tabular}} &  \multirow{2}*{\begin{tabular}{l} Std. Dev. \\  Width \end{tabular}}  & \multicolumn{2}{c}{ Points within (\%)} \\  
   \cmidrule{6-7} & & & & &  1SD/50P &  2SD/95P   \\
        \midrule
\multirow{4}{*}{10-fold}  
    &   INLA    &  Quantiles      & 0.023     & 0.058  & 6.021    & 45.288  \\
    & SpRF      &  Quantiles      & 0.092     & 0.141  & 69.11    & 87.435  \\
    \cdashline{2-7}
    & GPBoost   &  SD               & 0.136     & 0.013  & 84.293   & 95.55   \\
    & FRK       &  SD               & 0.099     & 0.077  & 97.644   & 98.953  \\
        \midrule
\multirow{4}{*}{50-fold}  
    &   INLA    &  Quantiles      & 0.094     & 0.162 & 22.251    & 46.073 \\
    & SpRF      &  Quantiles      & 0.075     & 0.116 & 62.827    & 89.529 \\
    \cdashline{2-7}
    & GPBoost   &  SD               & 0.112     & 0.014 & 81.152    & 91.361 \\
    & FRK       &  SD               & 0.063     & 0.068 & 94.764    & 98.953 \\        
		 \bottomrule
	\end{tabular} }
	\label{tab:intervalpredis_old}
\end{table}

\begin{figure}
    \centering

    \subfloat[][]{
        \includegraphics[width=0.4\textwidth]{figures/Old/Kenya_observations_cropped.png}
        \label{fig:Kenya_2009_prevalence}
    }\hspace{30px}
     \subfloat[][]{
        \includegraphics[width=0.4\textwidth]{figures/Old/Kenya_map_surface_cropped.png}
        \label{fig:Kenya_MAP_surface}
    } 
    \caption{2009 malaria prevalence data in Kenya. (a) shows prevalence survey results, while (b) shows the Malaria Atlas project predicted prevalence.}
    \label{fig:Kenya_data_old}
    
\end{figure}

\begin{figure}[!ht]
\centering

    \subfloat[][10-fold CV locations]{
        \includegraphics[width=0.35\textwidth]{figures/Old/10_folds_positions.png}
        \label{fig:10foldspos_old}
    }\hspace{40px}
     \subfloat[][50-fold CV locations]{
        \includegraphics[width=0.35\textwidth]{figures/Old/50_folds_positions.png}
        \label{fig:50foldspos_old}
    } 
    \caption{Malaria prevalence locations in Kenya for 2009. Colours represent different cross validation folds for 10 and 50-fold CV.  }
    \label{fig:cvpositions_old}
    
\end{figure}

\begin{figure}
    \centering
    \subfloat[][]{
        \includegraphics[width = 0.45\textwidth]{figures/OLD/Input_points_plots/observation.png}
        \label{fig:Africa_observation_points_old}
    }
    \subfloat[][]{
        \includegraphics[width = 0.45\textwidth]{figures/Old/Actual_Predicted_50fold_2.png}
        \label{fig:Africa_observation_binomial_points_old}
    }
    \\
    \subfloat[][]{
        \includegraphics[width = 0.45\textwidth]{figures/Old/Input_points_plots/uniform_simulated.png}
        \label{fig:Africa_uniform_binomial_points_old}
    }
    \subfloat[][]{
        \includegraphics[width = 0.45\textwidth]{figures/Old/Input_points_plots/MAP_surface.png}
        \label{fig:MAP_raster_old}
    }
    
   \caption{\textit{P. falciparum} prevalence data used to fit the 4 models at continental scale. \ref{fig:Africa_observation_points} shows the 2009 observed data at 942 locations. \ref{fig:Africa_observation_binomial_points} shows the prevalence generated from binomial samples at the observation locations. \ref{fig:Africa_uniform_binomial_points} shows the prevalence generated by binomial samples at 1000 uniformly selected locations. \ref{fig:MAP_raster} is the Malaria Atlas Project predicted prevalence raster from 2009 used to generate the samples in \ref{fig:Africa_observation_binomial_points} and \ref{fig:Africa_uniform_binomial_points}.}
   \label{fig:Africa_input_data_old}
\end{figure}

\begin{figure}[!p]
    \captionsetup{position = top}
    \centering
    \subfloat[][INLA]{
       \includegraphics[width = 0.7\textwidth]{figures/Old/prediction_maps/INLA_Kenya.png}
       \label{fig:INLA_Kenya_map_old}
    }\vspace{-10px}\\
    \subfloat[][SpRF]{
       \includegraphics[width = 0.7\textwidth]{figures/Old/prediction_maps/SpRF_Kenya.png}
       \label{fig:SpRF_Kenya_map_old}
    }\vspace{-10px}\\
    \subfloat[][GPBoost]{
       \includegraphics[width = 0.7\textwidth]{figures/Old/prediction_maps/GPBoost_Kenya.png}
       \label{fig:GPBoost_Kenya_map_old}
    }\vspace{-10px}\\
    \subfloat[][FRK]{
       \includegraphics[width = 0.7\textwidth]{figures/Old/prediction_maps/FRK_Kenya.png}
       \label{fig:FRK_Kenya_map_old}
    }
    \captionsetup{position = bottom}
    \caption{Predicted prevalences and uncertainties for the four models when trained on malaria prevalence data for Kenya in 2009. The uncertainties for INLA and SpRF are given as the interquartile range (IQR), and as the standard deviation (SD) for GPBoost and FRK.}
    \label{fig:Kenya_maps_old}
\end{figure}

\begin{figure}[!ht]
    \centering
     \subfloat[][INLA]{
        \includegraphics[width=0.48\textwidth]{figures/Old/INLA10_Intervals.png}
        \label{fig:INLA10_old}
    } 
    \subfloat[][SpRF]{
        \includegraphics[width=0.48\textwidth]{Figures/Old/SpRF10_Intervals.png}
        \label{fig:SpRF10_old}
    } \\
    \subfloat[][GPBoost]{
        \includegraphics[width=0.48\textwidth]{figures/Old/GPBoost10_Intervals.png}
        \label{fig:GPBoost10_old}
    } 
    \subfloat[][FRK]{
        \includegraphics[width=0.48\textwidth]{figures/Old/FRK10_Intervals.png}
        \label{fig:FRK10_old}
    } 
    \caption{Interval predictions for 10-fold cross validation.  }
    \label{fig:interval10fold1_old}
\end{figure}


\begin{figure}
\begin{tabular}{p{2mm}M{0.31\textwidth}M{0.31\textwidth}M{0.31\textwidth}}
        &  (i) Observation data& (ii) Binomial sampling at observation locations & (iii) Binomial sampling with uniform coverage \\
    \rotatebox[origin = c]{90}{(a) INLA} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_Observation_942_prevalence.png }
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_observation_locations_914_prevalence.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_uniform_1000_prevalence.png} \\
    \rotatebox[origin = c]{90}{(b) SpRF} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_Observation_942_prevalence.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_observation_locations_914_prevalence.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_uniform_1000_prevalence.png} \\
    \rotatebox[origin = c]{90}{(c) GPBoost} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_Observation_942_prevalence.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_observation_locations_914_prevalence.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_uniform_1000_prevalence.png} \\
    \rotatebox[origin = c]{90}{(d) FRK} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_Observation_942_prevalence.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_observation_locations_914_prevalence.png} &
    \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_uniform_1000_prevalence.png}
  
\end{tabular}
  
    \caption{\textit{P. falciparum} prevalence predictions when fit using three different datasets. In column (i), models are fitted using the survey data from Africa in 2009. In column (ii), binomial samples are drawn from the Malaria Atlas prevalence raster at the same survey locations. In column (iii), binomial samples are drawn using this raster at 1000 uniformly selected locations across the continent.}
    \label{fig:Africa_prevalence_maps_old}
\end{figure}


\begin{figure}
\begin{tabular}{p{2mm}M{0.31\textwidth}M{0.31\textwidth}M{0.31\textwidth}}
        &  (i) Observation data& (ii) Binomial sampling at observation locations & (iii) Binomial sampling with uniform coverage \\
    \rotatebox[origin = c]{90}{(a) INLA} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_Observation_942_uncertainty.png }
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_observation_locations_914_uncertainty.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/INLA_uniform_1000_uncertainty.png} \\
    \rotatebox[origin = c]{90}{(b) SpRF} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_Observation_942_uncertainty.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_observation_locations_914_uncertainty.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/SpRF_uniform_1000_uncertainty.png} \\
    \rotatebox[origin = c]{90}{(c) GPBoost} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_Observation_942_uncertainty.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_observation_locations_914_uncertainty.png} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/GPBoost_uniform_1000_uncertainty.png} \\
    \rotatebox[origin = c]{90}{(d) FRK} 
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_Observation_942_uncertainty.png}
    & \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_observation_locations_914_uncertainty.png} &
    \includegraphics[width=0.31\textwidth]{figures/Old/prediction_maps/Africa_Maps/FRK_uniform_1000_uncertainty.png}
  
\end{tabular}
  
    \caption{Prevalence uncertainties for each of the maps shown in Figure~\ref{fig:Africa_prevalence_maps}.}
    \label{fig:Africa_uncertainty_maps_old}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.9]{figures/Old/Actual_Predicted_2.png}
    \caption{Results of the four models using 10-fold CV.}
    \label{fig:actpreds10fold_old}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.9]{figures/Old/Actual_Predicted_50fold_2.png}
    \caption{Results of the four models using 50-fold CV with folds in different colours.}
    \label{fig:actpreds50fold_old}
\end{figure}

\begin{figure}[!ht]
    \subfloat[][Malaria prevalence]{
        \includegraphics[width=0.48\textwidth]{figures/Old/Prevalence.png}
        \label{fig:prev_old}
    }
     \subfloat[][Density of sampled locations]{
        \includegraphics[width=0.48\textwidth]{figures/Old/Density_map.png}
        \label{fig:density_old}
    }  
    \caption{Malaria prevalence in Kenya for 2009 and the kernel density estimates of the sampled locations.  }
    \label{fig:actualanddensityinmap_old}
\end{figure}


\begin{figure}[!ht]
    \subfloat[][10 folds]{
        \includegraphics[scale = 0.8]{figures/Old/density_prev_10folds.png}
        \label{fig:actualanddensity10folds_old}
    }
     \subfloat[][50 folds]{
        \includegraphics[scale = 0.8]{figures/Old/density_prev_50folds.png}
        \label{fig:actualanddensity50folds_old}
    }  
    \caption{Malaria prevalence and kernel density estimates of different clusters (folds) with zero prevalence observations taken out.  }
    \label{fig:actualanddensity_old}
\end{figure}



\begin{figure}[!ht]
    \centering
     \subfloat[][Density and absolute errors of the 4 models using 10-fold CV]{
        \includegraphics[scale = 0.65]{figures/Old/errors_density_10_fold.png}
        \label{fig:errordensity10folds_old}
    } \\
    \subfloat[][Density and absolute errors of the 4 models using 50-fold CV]{
        \includegraphics[scale = 0.7]{figures/Old/errors_density_50_fold.png}
        \label{fig:errordensity50folds_old}
    } 
    \caption{Kernel density estimates of the locations and the absolute errors of the 4 models for 10 and 50-fold cross validation.   }
    \label{fig:errordensity_old}
\end{figure}




\begin{figure}[!ht]
    \centering
     \subfloat[][INLA]{
        \includegraphics[width=0.48\textwidth]{figures/Old/INLA50_Intervals.png}
        \label{fig:INLA50_old}
    } 
    \subfloat[][SpRF]{
        \includegraphics[width=0.48\textwidth]{figures/Old/SpRF50_Intervals.png}
        \label{fig:SpRF50_old}
    } \\
    \subfloat[][GPBoost]{
        \includegraphics[width=0.48\textwidth]{figures/Old/GPBoost50_Intervals.png}
        \label{fig:GPBoost50_old}
    } 
    \subfloat[][FRK]{
        \includegraphics[width=0.48\textwidth]{figures/Old/FRK50_Intervals.png}
        \label{fig:FRK50_old}
    } 
    \caption{Interval predictions for 50-fold cross validation.  }
    \label{fig:interval50fold_old}
\end{figure}



\begin{figure}[!ht]
    \centering
     \subfloat[][Density and interval widths of the 4 models using 10-fold CV]{
        \includegraphics[scale = 0.65]{figures/Old/int_widths_density_10_fold.png}
        \label{fig:widthdensity10folds_old}
    } \\
    \subfloat[][Density and interval widths of the 4 models using 50-fold CV]{
        \includegraphics[scale = 0.7]{figures/Old/int_widths_density_50_fold.png}
        \label{fig:widthdensity50folds_old}
    } 
    \caption{Kernel density estimates of the locations and the interval widths of the 4 models for 10 and 50-fold cross validation.}
    \label{fig:widthdensity_old}
\end{figure}

